Simultaneously Achieving Sublinear Regret and Constraint Violations for Online Convex Optimization with Time-varying Constraints

In this paper, we develop a novel virtual-queue-based online algorithm for online convex optimization (OCO) problems with long-term and time-varying constraints and conduct a performance analysis with respect to the dynamic regret and constraint violations. We design a new update rule of dual variables and a new way of incorporating time-varying constraint functions into the dual variables. To the best of our knowledge, our algorithm is the first parameter-free algorithm to simultaneously achieve sublinear dynamic regret and constraint violations. Our proposed algorithm also outperforms the state-of-the-art results in many aspects, e.g., our algorithm does not require the Slater condition. Meanwhile, for a group of practical and widely-studied constrained OCO problems in which the variation of consecutive constraints is smooth enough across time, our algorithm achieves $O(1)$ constraint violations. Furthermore, we extend our algorithm and analysis to the case when the time horizon $T$ is unknown. Finally, numerical experiments are conducted to validate the theoretical guarantees of our algorithm, and some applications of our proposed framework will be outlined.

==> temp.tex <==
%table
\begin{center}
\small{
%\begin{sidewaystable}[htbp]
%\begin{table*}[htbp]
%\centering
\begin{adjustbox}{angle=90,caption={Comparison of performance bounds for OCO with long-term and time-varying constraints with respect to dynamic benchmark},float=table}
\begin{tabular}{cccccc}
\hline
Reference   &  Regret(R) &  Constraint violations(C)
& Parameter-free& Slater condition-free\protect\footnotemark & Simultaneous sublinear R\&C\\
\hline
      \cite{chen2017an} & $O(\max\{ { V }_{ x }{ T }^{ a },$
      \\
      &  ${ V }_{ g }{ T }^{ a },{ T }^{ 1-a }\} )$ & $O({ T }^{ 1-a })$ &\Checkmark & \XSolid &\XSolid\\
      \midrule
      \cite{chen2018heterogeneous} & $O({T}^{\frac{7}{8}}{V}_{x})$ & $O(\max\{{T}^{\frac{15}{16}},{T}^{\frac{7}{8}}{V}_{x}\})$ & \Checkmark &\Checkmark & \XSolid \\
     % & &  \small{${T}^{7/8}{V}_{x}\})$} \\
      \midrule
    \cite{chen2019bandit}   & $O({ V }_{ x }{ T }^{ \frac{3}{4} })$  &  $O({ T }^{\frac{3}{4} })$ &\Checkmark & \XSolid &\XSolid
      \\
      \midrule
     \cite{chen2019bandit}   & $O({ V }_{ x }{ T }^{ \frac{1}{2} })$  &  $O({ T }^{ \frac{1}{2} })$ &\Checkmark & \XSolid &\XSolid
      \\
      \midrule
     \cite{cao2018online}  & $O({ V }_{ x }^{ \frac{1}{2} }{ T }^{ \frac{1}{2} })$  & $O({ V }_{ x }^{ \frac{1}{4} }{ T }^{ \frac{3}{4} })$ &\XSolid  & \XSolid &\Checkmark
      \\
      \midrule
    % \small{ \textcolor{red}{\cite{cao2018online}}}  & \small{$O({ V }_{ x }{ T }^{ 1/2 })$}  & \small{ $O(max\{{ T }^{ 3/4 } )$} &\small{\Checkmark}  & \small{\Checkmark}  &\small{\XSolid}
     % \\
     % &  & \small{$,{ V }_{ x }^{ 1/2 }{ T }^{ 1/2 }\}$} \\
     % \midrule
      This work(Thm.1) & $O(\max\{ \sqrt { T{ V }_{ x } } ,{ V }_{ g }\} )$ & $O(\max\{ \sqrt { T } ,{ V }_{ g }\} )$ & \Checkmark & \Checkmark & \Checkmark
      \\
      \midrule
     This work(Thm.1)& $O( \sqrt { T{ V }_{ x } } )$ & $O(\max\{ {T}^{\frac{3}{4}} ,{ V }_{ g }\} )$ & \Checkmark & \Checkmark & \Checkmark\\
\hline
\end{tabular}
\label{tab:plain}
%\caption{ Comparison of performance bounds for OCO with long-term and time-varying constraints with respect to dynamic benchmark}
%\end{sidewaystable}
\end{adjustbox}
%\end{table*}
}
\end{center}
%\footnotetext{Slater condition-free means without requiring Slater condition holds and [3] assumes a slightly stronger Slater condition.}
\footnotetext{[3] assumes a slightly stronger Slater condition.} 


In this paper, we develop a novel virtual-queue-based online algorithm for online convex optimization (OCO) problems with long-term and time-varying constraints
and conduct a performance analysis with respect to the dynamic regret and constraint violations. We design a new update rule of dual variables and a new way of incorporating time-varying constraint functions into the dual variables. To the best of our knowledge, our algorithm is the first parameter-free algorithm to simultaneously achieve sublinear dynamic regret and constraint violations. Our proposed algorithm also outperforms the state-of-the-art results in many aspects, e.g., our algorithm does not require the Slater condition. Meanwhile, for a group of practical and widely-studied constrained OCO problems in which the variation of consecutive constraints is smooth enough across time, our algorithm achieves $O(1)$ constraint violations. Furthermore, we extend our algorithm and analysis to the case when the time horizon $T$ is unknown. Finally, numerical experiments are conducted to validate the theoretical guarantees of our algorithm, and some applications of our proposed framework will be outlined.
